Beyond Color and Lines: Zero-Shot Style-Specific Image Variations with Coordinated Semantics

Traditionally, style has been primarily considered in terms of artistic elements such as colors, brushstrokes, and lighting. However, identical semantic subjects, like people, boats, and houses, can vary significantly across different artistic traditions, indicating that style also encompasses the underlying semantics. Therefore, in this study, we propose a zero-shot scheme for image variation with coordinated semantics. Specifically, our scheme transforms the image-to-image problem into an image-to-text-to-image problem. The image-to-text operation employs vision-language models e.g., BLIP) to generate text describing the content of the input image, including the objects and their positions. Subsequently, the input style keyword is elaborated into a detailed description of this style and then merged with the content text using the reasoning capabilities of ChatGPT. Finally, the text-to-image operation utilizes a Diffusion model to generate images based on the text prompt. To enable the Diffusion model to accommodate more styles, we propose a fine-tuning strategy that injects text and style constraints into cross-attention. This ensures that the output image exhibits similar semantics in the desired style. To validate the performance of the proposed scheme, we constructed a benchmark comprising images of various styles and scenes and introduced two novel metrics. Despite its simplicity, our scheme yields highly plausible results in a zero-shot manner, particularly for generating stylized images with high-fidelity semantics.

==> dataset.tex <==
\section{Details of Dataset ZsSTD}

We created a dataset containing 5,710 images exhibiting various artistic styles sourced from WikiArt \cite{phillips2011wiki} and the wider web. The ZsSTD encompasses \textbf{7} distinct styles: 'realist oil painting,' 'anime,' 'Chinese ink painting,' 'impressionist oil painting,' 'abstract painting,' 'Chinese freehand painting,' and 'real photographs.' Each style category contains a substantial number of images, all accompanied by meticulously annotated text descriptions to ensure accurate representation, eschewing reliance on conventional image-to-text methods. Figure 1 shows the dataset directory and several samples, while Table \ref{tabel:dataset} details the distribution of images across the different style categories within our newly compiled dataset.



%\begin{figure*}[t]
%\centering
%\includegraphics[width=1\textwidth]{figure/dataset.png} 
%\caption{(a) The directory of our new dataset ZsSTD, including images and descriptive annotation files. (b) Partial data on impression-style oil paintings. (c) Annotation file for the text description corresponding to the impression style oil painting. (d)Partial data on Chinese freehand art style.}
%\label{fig:dataset}
%\end{figure*}


\begin{table}[H]
\caption{The detailed information of ZsSTD.}
\label{tabel:dataset}
\begin{tabular}{c|cc}
\hline
Style & Num of Data & Num of Subcategories\\ 
\hline
Realistic          & 804            & 3                                                                     \\
Impression         & 908              & 3                                                                     \\
Abstract           & 965              & 5                                                                     \\
Ink paintings      & 1021             & 0                                                                     \\
Chinese freehand   & 940              & 3                                                                     \\
Anime              & 1072             & 3  \\
\hline
\textbf{Total }    & \textbf{5710}    & -                                                                     \\ \hline
\end{tabular}
\end{table}

==> moreRes.tex <==
\section{More Experimental Results}

\subsection{Image Variation Results}

In our experiment, we used each image from a distinct style within the new ZsSTD dataset as input, transforming them into six different styles, each directed by a unique textual style prompt. Notably, we excluded abstract styles as inputs and did not generate real photos as outputs. The experimental results are displayed in Figure 2 and Figure 3. As illustrated in Figure 2, our innovative approach effectively generates image variations by distinctly utilizing concise text prompts as style directives.

% in contrast to the baseline method, which depends on carefully curated, style-aligned images as prompts.

As seen in Figure2 and Figure 3, the image quality generated by our method is notably high. The objects depicted within the figures are harmoniously aligned with the cultural and stylistic contexts, creating a vivid narrative reminiscent of a painting that unfolds diverse worlds, each telling the same stories in unique ways. These results include a wide array of concrete objects, such as bridges, towering skyscrapers, and intricate pathways, all of which are naturally influenced by various styles, cultures, and artistic forms, leading to varied expressions. As illustrated in Figure 2, our outcomes seamlessly integrate these objects with the selected style, ensuring a cohesive and contextually appropriate presentation.


%\begin{figure*}[tbh]
%\centering
%\includegraphics[width=0.9\textwidth]{figure/more_results.png} 
%\caption{More image variation results obtained by our method. Enlarging the image reveals clear stylistic features.}
%\label{moreresults}
%\end{figure*}

\begin{table*}[bt]
\tiny
\setlength{\tabcolsep}{0.5mm}
\caption{The quantitative results of our method and style transfer baselines.}
\label{quantCompar}
\begin{tabular}{c|ccccc|cccccc|cccccc|cccccc|cccccc}
\hline

 & \multicolumn{5}{c|}{\cellcolor{pearl}{Realistic oil}} 
& & \multicolumn{5}{c|}{\cellcolor{pastelyellow}{Abstract}}     
& & \multicolumn{5}{c|}{\cellcolor{pink}{Ink painting}}   
& & \multicolumn{5}{c|}{\cellcolor{myorange}{Impression}}  
& & \multicolumn{5}{c}{\cellcolor{babyblue}{Anime}}  \\ 

\hline

\cellcolor{pink}{Ink painting} 
\rowcolor{aliceblue}
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &
& Ours & Avatar & AdaIn & Artflow & styTR & 
& Ours & Avatar & AdaIn & Artflow & styTR
\\ \cline{1-30}

SML$\downarrow$ & 
\Ud{6.56} & 7.72 & 7.15 & 6.91 & \textbf{5.72} &  & 
\textbf{5.01} & 8.06 & 9.62 & \Ud{6.18} & 7.45 &  & 
- & - & - & - & - &  & 
7.23 & \Ud{6.38} & 7.96 & 8.01 & \textbf{6.12} &  & 
6.95 & 6.83 & 7.21 & \Ud{6.55} & \textbf{5.97} \\

CMS$\uparrow$ &
\textbf{0.813} & 0.325 & 0.245 & \Ud{0.357} & 0.163 &  & 
\textbf{0.315} & 0.132 & 0.095 & 0.119 & \Ud{0.217} &  & 
- & - & - & - & - &  & 
\textbf{0.678} & 0.275 & 0.193 & \Ud{0.326} & 0.242 &  & 
\textbf{0.484} & 0.254 & 0.140 & 0.239 & \Ud{0.384} \\

FID$\downarrow$ & 
\textbf{14.48} & 17.61 & 16.32 & 16.73 & \Ud{15.41} &  & 
\textbf{18.35} & 22.78 & 21.31 & \Ud{19.98} & 20.64 &  & 
- & - & - & - & - &  & 
16.91 & 18.73 & 17.82          & \textbf{14.55} & \Ud{15.76} &  & 
\Ud{15.43} & 25.00 & \textbf{14.99} & 18.76          & 22.32 \\

CLIPS$\uparrow$  &
\Ud{24.37}     & 23.98 & 24.12 & \textbf{25.72} & 23.41 &  & 
\textbf{24.11} & \Ud{19.54} & 18.96 & 19.12 & 18.74 &  &
- & - & - & - & - &  &
\textbf{26.98} & \Ud{23.57} & 23.61 & 21.73 & 20.73 &  & 
23.41          & \textbf{26.73}& 25.66 & \Ud{26.45} & 24.56 \\ \hline

\cellcolor{celadon}{Photo}
\rowcolor{aliceblue}
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &
& Ours & Avatar & AdaIn & Artflow & styTR & 
& Ours & Avatar & AdaIn & Artflow & styTR
\\ \cline{1-30}

SML$\downarrow$ & 
6.87 & \Ud{5.48} & 6.01 & 6.27 & \textbf{4.75} &  & 
\textbf{6.99} & 8.35 & 9.15 & \Ud{7.92} & 8.63 &  & 
\textbf{4.82} & 5.91 & \Ud{5.25} & 6.41 & 5.37 &  & 
7.74 & 6.42 & 8.62 & \Ud{6.17} & \textbf{5.86} &  & 
6.31 & \textbf{5.27} & 6.29 & \Ud{5.88} & 6.16 \\

CMS $\uparrow$&
0.672 & \textbf{0.817} & 0.625          & 0.752      & \Ud{0.801} &  & 
0.432 & 0.527          & \textbf{0.641} & 0.146      & \Ud{0.599} &  & 
0.514 & 0.468          & 0.385          & \Ud{0.548} & \textbf{0.624} &  & 
\textbf{0.753}         & 0.519          & 0.456 & \Ud{0.620} & 0.572 &  & 
0.581 & \Ud{0.622} & 0.196 & 0.426 & \textbf{0.728} \\

FID$\downarrow$ &
\Ud{16.90} & \textbf{16.21} & 20.78          & 18.89          & 24.98 &  &
\textbf{19.21} & 26.56 & 26.34          & \Ud{22.12}          & 23.90 &  &
\textbf{15.67} & 22.09 & 20.89          & 19.32          & \Ud{16.25} & &
17.98          & 26.78 & 16.78          & \Ud{16.21}     & \textbf{14.78} &  & 
18.32          & 21.92 & 21.33          & \textbf{15.43} & \Ud{17.43} \\

CLIPS $\uparrow$&
\textbf{29.68} & 27.43          & \Ud{28.75} & 23.45 & 28.69 &  &
\textbf{28.43} & 20.78          & \Ud{22.94} & 21.11 & 21.39 &  &
\textbf{29.41} & \Ud{23.3}       & 22.71 & 20.19 & 22.49 &  &
\textbf{28.89} & \Ud{26.77}     & 24.59 & 26.21 & 23.99 &  & 
\Ud{27.33}     & \textbf{28.93} & 26.43 & 24.86 & 25.52 \\ \hline


\cellcolor{babyblue}{Anime}
\rowcolor{aliceblue}
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &  
& Ours & Avatar & AdaIn & Artflow & styTR &
& Ours & Avatar & AdaIn & Artflow & styTR & 
& Ours & Avatar & AdaIn & Artflow & styTR
\\ \cline{1-30}

SML$\downarrow$ & 
\textbf{6.41} & 8.26 & 7.77 & \Ud{6.92} & 7.12 &  & 
\textbf{6.48} & 10.01 & 9.87 & \Ud{8.51} & 9.66 &  & 
\textbf{5.52} & 8.91 & 9.03 & 7.84 & \Ud{6.69} &  & 
\Ud{5.76} & 6.71 & 8.30 & 6.72 & \textbf{5.42} &  & 
- & - & - & - & -  \\

CMS$\uparrow$ &
0.519 & 0.451 & 0.426 & \Ud{0.525} & \textbf{0.539} &  & 
\Ud{0.432} & \textbf{0.513} & 0.289 & 0.371 & 0.106 &  & 
\textbf{0.686} & 0.364 & 0.239 & 0.181 & \Ud{0.524} &  &
\Ud{0.586} & \textbf{0.653} & 0.327 & 0.274 & 0.295 &  & 
- & - & - & - & -  \\

FID $\downarrow$&
15.79 & 18.91 & 19.32 & \Ud{15.22} & \textbf{14.76} &  &
19.32 & \Ud{19.23} & \textbf{16.78} & 22.45   & 20.89 &  & 
\textbf{18.91} & 24.12  & 23.56 & 21.01   & \Ud{19.24} &  &
\textbf{14.10} & 22.67 & 23.12 & 19.21 & \Ud{15.67} &  & 
- & - & - & - & - \\

CLIPS$\uparrow$&
\Ud{26.53} & 24.56 & \textbf{26.87} & 25.43 & 24.66 &  &
\textbf{29.09} & 21.35 & \Ud{22.04} & 20.68 & 21.16 &  &
\textbf{28.76} & 21.45 & \Ud{24.33} & 23.34 & 22.07 &  &
\textbf{29.47} & \Ud{27.33} & 26.42 & 27.32 & 25.88 &  & 
- & - & - & - & - \\ \hline

\end{tabular}
\end{table*}



\begin{table*}[bt]
\tiny
\setlength{\tabcolsep}{0.5mm}
\caption{The quantitative results of our method and multi-conditional image generation baselines.}
\label{quantComparGen}
\begin{tabular}{c|ccccc|ccccc|ccccc}
\hline

& \multicolumn{5}{c|}{\cellcolor{pearl}{Realistic oil}}   
& \multicolumn{5}{c|}{\cellcolor{myorange}{Impression}}  
& \multicolumn{5}{c}{\cellcolor{babyblue}{Anime}}  \\ 

\hline

\cellcolor{celadon}{Photo}
\rowcolor{aliceblue}
& Ours & styleCLIP & CLIPstyler & TextInversion(SD) & Dreambooth(SD) &  
Ours & styleCLIP & CLIPstyler & TextInversion(SD) & Dreambooth(SD) &  
Ours & styleCLIP & CLIPstyler & TextInversion(SD) & Dreambooth(SD)
\\ 
\cline{1-16}

SML$\downarrow$ & 
\Ud{6.87} & 7.23 & 8.92 & 7.63 & \textbf{6.25} &
7.74 & 7.77 & 9.67 & \Ud{7.42} & \textbf{5.98} & 
\Ud{6.31} & 7.56 & 8.48 & \textbf{5.98} & 8.2
\\

CMS $\uparrow$&
\textbf{0.67} & 0.37 & \Ud{0.57} & 0.30 & 0.31 & 
\textbf{0.75} & \Ud{0.51} & 0.38 & 0.58 & 0.22 & 
\textbf{0.58} & \Ud{0.44} & 0.40 & 0.38 & 0.34\\

FID$\downarrow$ &
\textbf{16.90} & \Ud{18.58} & 19.21 & 19.21 & 19.99 & 
\textbf{17.98} & 19.49 & 21.63 & \Ud{19.19} & 21.42 & 
\textbf{18.32} & 20.49 & 30.17 & \Ud{20.04} & 20.9 \\

CLIPS $\uparrow$&
\textbf{29.68} & 21.36 & 20.01 & 25.92 & \Ud{26.15} &
\textbf{28.89} & 20.82 & 17.69 & 24.52 & \Ud{27.56} & 
\textbf{27.33} & 20.04 & 20.74 & 23.42 & \Ud{25.52}
\\ \hline

\end{tabular}
\end{table*}



\subsection{Qualitative Comparison}

We compare our method to \textbf{12} baselines across three categories of tasks with similar focuses: (i) image-driven style transfer methods, including: CNN-based method Avatar \cite{sheng2018avatar}, AdaIn \cite{huang2017arbitrary}, flow-based method ArtFlow \cite{li2021multi}, and Transformer method styTR \cite{deng2022stytr2}; (ii) text-driven style transfer tasks, such as styleGAN-NADA \cite{gal2022stylegan}, styleCLIP \cite{patashnik2021styleclip}, CLIPstyler \cite{kwon2022clipstyler}, VQGAN-CLIP \cite{crowson2022vqgan}; and (iii) multi-conditional image generation methods, including Ernie \cite{sun2019ernie}, SD-XL Refiner \cite{podell2023sdxl}, ControNet \cite{zhang2023adding}, and Dreambooth \cite{ruiz2023dreambooth}. More results are shown in Figures 4, 5 and 6.

Figures 4, 5 and 6 indicate that style transfer methods struggle with input images that have distinct styles, often resulting in issues like color bleeding and style overlay, which degrade image quality. Furthermore, when the content and style of an image do not blend seamlessly, the faithfulness of the generated image is compromised. As for multi-conditional generation methods, the results reveal that existing approaches often struggle to capture the finer details of image content, resulting in a noticeable semantic deviation between the generated images and their originals. Furthermore, these methods exhibit significant limitations in producing multiple styles, particularly when dealing with abstract styles and Chinese ink paintings, where they frequently fail to generate images that accurately reflect the desired style.

\subsection{Quantitative Comparison}
Tables 2 and 3 present the scores for our method and various baselines, including image-driven style transfer methods, text-driven transfer methods, and multi-conditional image generation methods. It should be noted that we have restricted our evaluation to styles that are compatible with all baseline methods to ensure a fair comparison. Table \ref{quantCompar} shows that our method performs competitively with image-driven style transfer methods in terms of both content and style, despite these methods' emphasis on minimizing both content and style loss. Furthermore, Table \ref{quantComparGen} demonstrates that our method outperforms all baselines in terms of content, image quality, and the overall accuracy and coherence of the image’s stylistic portrayal. Although the SML scores for our method are not the highest, they remain closely aligned with those of the baselines.




